Probabilistic Forecasting of the Masses and Radii of Other Worlds

Mass and radius are two of the most fundamental properties of an astronomical object. Increasingly, new planet discoveries are being announced with a measurement of one of these terms, but not both. This has led to a growing need to forecast the missing quantity using the other, especially when predicting the detectability of certain follow-up observations. We present am unbiased forecasting model built upon a probabilistic mass-radius relation conditioned on a sample of 316 well-constrained objects. Our publicly available code, Forecaster, accounts for observational errors, hyper-parameter uncertainties and the intrinsic dispersions observed in the calibration sample. By conditioning our model upon a sample spanning dwarf planets to late-type stars, Forecaster can predict the mass (or radius) from the radius (or mass) for objects covering nine orders-of-magnitude in mass. Classification is naturally performed by our model, which uses four classes we label as Terran worlds, Neptunian worlds, Jovian worlds and stars. Our classification identifies dwarf planets as merely low-mass Terrans (like the Earth), and brown dwarfs as merely high-mass Jovians (like Jupiter). We detect a transition in the mass-radius relation at $2.0_{-0.6}^{+0.7} M_\oplus$, which we associate with the divide between solid, Terran worlds and Neptunian worlds. This independent analysis adds further weight to the emerging consensus that rocky Super-Earths represent a narrower region of parameter space than originally thought. Effectively, then, the Earth is the Super-Earth we have been looking for.

==> journals.tex <==
%\newcommand{\aj}{{\it AJ}}%
          % Astronomical Journal
\newcommand{\actaa}{{\it Acta Astron.}}%
          % Acta Astronomica
%\newcommand{\araa}{{\it ARA\&A}}%
          % Annual Review of Astron and Astrophys
%\newcommand{\apj}{{\it ApJ}}%
          % Astrophysical Journal
%\newcommand{\apjl}{{\it ApJ}}%
          % Astrophysical Journal, Letters
%\newcommand{\apjs}{{\it ApJS}}%
          % Astrophysical Journal, Supplement
%\newcommand{\ao}{{\it Appl.~Opt.}}%
          % Applied Optics
%\newcommand{\apss}{{\it Ap\&SS}}%
          % Astrophysics and Space Science
%\newcommand{\aap}{{\it A\&A}}%
          % Astronomy and Astrophysics
%\newcommand{\aapr}{{\it A\&A~Rev.}}%
          % Astronomy and Astrophysics Reviews
%\newcommand{\aaps}{{\it A\&AS}}%
          % Astronomy and Astrophysics, Supplement
%\newcommand{\azh}{{\it AZh}}%
          % Astronomicheskii Zhurnal
%\newcommand{\baas}{{\it BAAS}}%
          % Bulletin of the AAS
\newcommand{\caa}{{\it Chinese Astron. Astrophys.}}%
  % Chinese Astronomy and Astrophysics
\newcommand{\cjaa}{{\it Chinese J. Astron. Astrophys.}}%
  % Chinese Journal of Astronomy and Astrophysics
%\newcommand{\icarus}{{\it Icarus}}%
  % Icarus
\newcommand{\jcap}{{\it J. Cosmology Astropart. Phys.}}%
  % Journal of Cosmology and Astroparticle Physics
%\newcommand{\jrasc}{{\it JRASC}}%
          % Journal of the RAS of Canada
%\newcommand{\memras}{{\it MmRAS}}%
          % Memoirs of the RAS
%\newcommand{\mnras}{{\it MNRAS}}%
          % Monthly Notices of the RAS
\newcommand{\na}{{\it New A}}%
  % New Astronomy
\newcommand{\nar}{{\it New A Rev.}}%
  % New Astronomy Review
%\newcommand{\pra}{{\it Phys.~Rev.~A}}%
          % Physical Review A: General Physics
%\newcommand{\prb}{{\it Phys.~Rev.~B}}%
          % Physical Review B: Solid State
%\newcommand{\prc}{{\it Phys.~Rev.~C}}%
          % Physical Review C
%\newcommand{\prd}{{\it Phys.~Rev.~D}}%
          % Physical Review D
%\newcommand{\pre}{{\it Phys.~Rev.~E}}%
          % Physical Review E
%\newcommand{\prl}{{\it Phys.~Rev.~Lett.}}%
          % Physical Review Letters
\newcommand{\pasa}{{\it PASA}}%
  % Publications of the Astron. Soc. of Australia
%\newcommand{\pasp}{{\it PASP}}%
          % Publications of the ASP
%\newcommand{\pasj}{{\it PASJ}}%
          % Publications of the ASJ
%\newcommand{\qjras}{{\it QJRAS}}%
          % Quarterly Journal of the RAS
\newcommand{\rmxaa}{{\it Rev. Mexicana Astron. Astrofis.}}%
  % Revista Mexicana de Astronomia y Astrofisica
%\newcommand{\skytel}{{\it S\&T}}%
          % Sky and Telescope
%\newcommand{\solphys}{{\it Sol.~Phys.}}%
          % Solar Physics
%\newcommand{\sovast}{{\it Soviet~Ast.}}%
          % Soviet Astronomy
%\newcommand{\ssr}{{\it Space~Sci.~Rev.}}%
          % Space Science Reviews
%\newcommand{\zap}{{\it ZAp}}%
          % Zeitschrift fuer Astrophysik
%\newcommand{\nat}{{\it Nature}}%
          % Nature
%\newcommand{\iaucirc}{{\it IAU~Circ.}}%
          % IAU Cirulars
%\newcommand{\aplett}{{\it Astrophys.~Lett.}}%
          % Astrophysics Letters and Communications
%\newcommand{\apspr}{{\it Astrophys.~Space~Phys.~Res.}}%
          % Astrophysics Space Physics Research
%\newcommand{\bain}{{\it Bull.~Astron.~Inst.~Netherlands}}%
          % Bulletin Astronomical Institute of the Netherlands
%\newcommand{\fcp}{{\it Fund.~Cosmic~Phys.}}%
          % Fundamental Cosmic Physics
%\newcommand{\gca}{{\it Geochim.~Cosmochim.~Acta}}%
          % Geochimica Cosmochimica Acta
%\newcommand{\grl}{{\it Geophys.~Res.~Lett.}}%
          % Geophysics Research Letters
%\newcommand{\jcp}{{\it J.~Chem.~Phys.}}%
          % Journal of Chemical Physics
%\newcommand{\jgr}{{\it J.~Geophys.~Res.}}%
          % Journal of Geophysical Research
%\newcommand{\jqsrt}{{\it J.~Quant.~Spec.~Radiat.~Transf.}}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
%\newcommand{\memsai}{{\it Mem.~Soc.~Astron.~Italiana}}%
          % Mem. Societa Astronomica Italiana
%\newcommand{\nphysa}{{\it Nucl.~Phys.~A}}%
          % Nuclear Physics A
%\newcommand{\physrep}{{\it Phys.~Rep.}}%
          % Physics Reports
%\newcommand{\physscr}{{\it Phys.~Scr}}%
          % Physica Scripta
%\newcommand{\planss}{{\it Planet.~Space~Sci.}}%
          % Planetary Space Science
%\newcommand{\procspie}{{\it Proc.~SPIE}}%
          % Proceedings of the SPIE
